Fixing Vulnerabilities Potentially Hinders Maintainability

Security is a requirement of utmost importance to produce high-quality software. However, there is still a considerable amount of vulnerabilities being discovered and fixed almost weekly. We hypothesize that developers affect the maintainability of their codebases when patching vulnerabilities. This paper evaluates the impact of patches to improve security on the maintainability of open-source software. Maintainability is measured based on the Better Code Hub's model of 10 guidelines on a dataset, including 1300 security-related commits. Results show evidence of a trade-off between security and maintainability for 41.90% of the cases, i.e., developers may hinder software maintainability. Our analysis shows that 38.29% of patches increased software complexity and 37.87% of patches increased the percentage of LOCs per unit. The implications of our study are that changes to codebases while patching vulnerabilities need to be performed with extra care; tools for patch risk assessment should be integrated into the CI/CD pipeline; computer science curricula needs to be updated; and, more secure programming languages are necessary.

==> Makefile <==
NAME:=emse20
REVISION=ba3364280bab9782adbc52f12ff813e5aeb30f9d

# To update, run: latex-process-inputs -makefilelist main.tex
TEX_FILES = \
$(NAME).tex

.DEFAULT_GOAL := pdf

pdf:
	latexmk -bibtex -pdf $(NAME)

final: pdf
	@echo '******** Did you spell-check the paper? ********'
	pdffonts $(NAME).pdf; fi
	
diff:
	git show $(REVISION):./$(NAME).tex > old.tex
	latexdiff old.tex emse20.tex > diff.tex
	latexmk diff.tex
	latexmk -c diff.tex
	rm old.tex diff.tex

clean:
	rm *aux *bbl *blg *log $(NAME).pdf *.fdb_latexmk *.synctex.gz *.fls *.out

read:
	evince $(NAME).pdf

tags: TAGS
TAGS: ${TEX_FILES}
	etags ${TEX_FILES}
